The Boomerang protocol: A Decentralised Privacy-Preserving Verifiable Incentive Protocol

In the era of data-driven economies, incentive systems and loyalty programs, have become ubiquitous in various sectors, including advertising, retail, travel, and financial services. While these systems offer advantages for both users and companies, they necessitate the transfer and analysis of substantial amounts of sensitive data. Privacy concerns have become increasingly pertinent, necessitating the development of privacy-preserving incentive protocols. Despite the rising demand for secure and decentralised systems, the existing landscape lacks a comprehensive solution. In this work, we propose the BOOMERANG protocol, a novel decentralised privacy-preserving incentive protocol that leverages cryptographic black box accumulators to securely and privately store user interactions within the incentive system. Moreover, the protocol employs zero-knowledge proofs to transparently compute rewards for users, ensuring verifiability while preserving their privacy. To further enhance public verifiability and transparency, we utilise a smart contract on a Layer 1 blockchain to verify these zero-knowledge proofs. The careful combination of black box accumulators and zero-knowledge proofs makes the BOOMERANG protocol highly efficient.

==> blockchain.tex <==
\section{Proof Verification via Smart Contracts}\label{sec:blockchain}

While computing the rewards proof and the proof of identity locally on device of the
user, the verification of the proofs need to be deliberately thought through. Anyone
that has access to the public parameters and the statement to be proven, can verify a
zero knowledge proof. However, an efficient form of public verifiability of the reward
computation can be achieved by verifying these proofs in a smart contract by a public
L1 blockchain. Additionally, this approach allows to perform the settlement of the
rewards payment for the incentive system also directly with the smart contract, by
transferring a cryptocurrency token to the user's wallet. The cryptocurrency token is
dependent on the underlying blockchain and the support for tokens within the smart
contract.

%\subsection{Challenges of Verifying Zero-Knowledge Proofs in a Smart Contract}
Yet, verifying zero-knowledge proofs (ZKPs) within smart contracts presents several
challenges. Firstly, the computational complexity of ZKPs can strain the limited computational
resources of smart contracts, potentially causing delays or higher gas costs. Scalability becomes
an issue when large data or complex computations are involved, impacting the overall transaction
throughput. Auditing and verifying the correctness and security properties of ZKPs require
expertise and can be time-consuming. Furthermore, upgradability and standardisation pose challenges
in keeping smart contracts aligned with evolving ZKP protocols. Addressing these challenges is
crucial to enable efficient and secure verification of ZKPs in smart contract environments.

\subsection{Smart Contract ZKP Verification at Scale}
For incentive systems with a large scale of users, the scalability issues can easily become a
problematic bottleneck. Fortunately, there are several solutions to address this issues.

\paragraph{Proof Aggregation.} In the scenario of multiple instances of the same proof, or if
multiple users are involved, proof aggregation can be used to improve the efficiency and reduce
the computational complexity. This can be achieved by leveraging the structure and the properties of
the underlying zero-knowledge proof scheme by combining multiple individual proofs to one larger
single proof. For the \protocolname protocol, multiple rewards proofs can be combined to create one
larger proof that can then be verified by the smart contract.

\paragraph{Batch Verification.} Given a large number of proofs that share similar computations or
properties, efficiency can significantly be improved using batch verification. Therefore, multiple
individual proofs are batched together and verified simultaneously. In the \protocolname protocol
numerous users submit similar reward proofs that can be processed in batches instead of individual
verification.

\paragraph{ZKRollups.}
Initially proposed by Whitehat~\cite{Whitehat2019}, zero-knowledge rollups are a
solution for the scalability problems in Ethereum. The idea is to move computation off-chain
and only perform minimal computations on-chain. For the \protocolname protocol, this could
be to process a batch of reward proof verifications off-chain and then performing a cryptographic
validity proof that the batch has been verified.

\paragraph{Partial Proof Verification.} Smart contracts are often computationally limited, and
depending on the zero-knowledge proof system and the complexity of the statements to be
proven the verification can be a complex task to perform. An efficient solution to has been
proposed as the Refereed Delegation of Computation (RDoC) protocol~\cite{CANETTI201316}.
The protocol has been adapted to efficiently verify zero-knowledge proofs in smart contracts on
Ethereum by Truebit~\cite{Truebit2017}.

The protocol works as follows; A prover computes a zero-knowledge proof about a statement
and sends it to the verifier. The verifier adds the proof to a smart contract that simply stores the
proof. The verifier can then complain to the smart contract and claim the proof is invalid. Next,
the smart contract lays out the verification circuit and the verifier sends the output of a chosen
gate in the circuit. The smart contract then uses binary search to identify the specific gate in
the circuit where the proofs diverge, and only needs to verify one single gate to determine if
the verifier or the prover is correct. The protocol has one complication, as how often a verifier
disagrees with the proof of the prover and if a prover should verify the proof at all, also known as
the verifiers dilemma~\cite{CCS:LTKS15}. However, this can be solved by incentivising the
verifiers to occasionally performing the verification.

%\subsection{Settlement}
%\todo[inline]{TODO some text about how tokens can be used for payment for the rewards/incentives. To clarify: Are new BAT tokens minted/generated freshly for rewards or are they just reassigned from a pool of tokens?}.


==> comparison.tex <==
\begin{landscape}
\section{Comparison of privacy-preserving incentive schemes}\label{app:comparison}

Table~\ref{tab:comparison} provides a comparison for privacy-focused incentive
schemes.

%Privacy pass~\cite{PoPETS:DGSTV18}
%Black box accumulators~\cite{PoPETS:JagRup16}
%BBA+~\cite{CCS:HHNR17}
%Adnostic~\cite{NDSS:TNBNB10} - only browser extension/hard to compare
%Privad~\cite{guha2009} - only browser extension/hard to compare
%P4TC~\cite{EPRINT:FHNRS18}
%BBW~\cite{PoPETS:HKRR20}


\begin{table}[!htb]
  \centering
  \caption{Comparison of privacy-preserving incentive schemes. Time issuing phase (IP), Time collection phase (CP), spending/verification phase (SVP) in $\SI{}{\milli}{\second}$.}
   \label{tab:comparison}
   \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccc}
        \toprule
        \multicolumn{6}{c}{Incentive schemes} \\
        ~ & Privacy pass~\cite{PoPETS:DGSTV18, challenge-bypass}
        & Black box accumulators~\cite{PoPETS:JagRup16}
        & BBA+~\cite{CCS:HHNR17}
        & BBW~\cite{PoPETS:HKRR20}
        & this work \\
        \midrule
        time (IP) & 2.6 & 36 & 11  & 72 & 4.52 \\
        time (CP) & 3.1 & 268 & 386 & 107 & 8.78 \\
        time (SVP) & 0.06 & 256 & 376  & 304 & 57.8 \\
        \midrule
        data (IP)  & ~ & 3kB & 1kB & 1kB & 10.9kB \\
        data (CP)  & ~ & 2kB & 4kB & 1.7kB & 25.2kB \\
        data (SVP)  & ~ & 1B & 14.3kB & 3.9kB & 152.9kB \\
        \midrule
        tokens & blinded tokens & SXDH-based commitments~\cite{EC:GroSah08} & structure-preserving trapdoor commitments~\cite{EC:AKOT15} & Pedersen commitments & Pedersen commitments/CurveTrees~\cite{EPRINT:CamHal22,291060} \\
        zkp & DLEQ & Groth-Sahai~\cite{EC:GroSah08} & Groth-Sahai~\cite{EC:GroSah08} &  Bulletproofs~\cite{SP:BBBPWM18}, $\Sigma$ proofs & Bulletproofs~\cite{SP:BBBPWM18}, $\Sigma$ proofs \\
        signatures & HMAC/SHA512 & Structure Preserving Signatures~\cite{C:AGHO11} & Structure Preserving Signatures~\cite{C:AGHO11} & Baldimtsi and Lysyanskaya~\cite{CCS:BalLys13} & Baldimtsi and Lysyanskaya~\cite{CCS:BalLys13} \\
        elliptic curves & curve25519~\cite{PKC:Bernstein06} & Barreto-Naehrig~\cite{SAC:BarNae05} & Barreto-Naehrig~\cite{SAC:BarNae05} &  curve25519~\cite{PKC:Bernstein06} & secp256r1 \\
        %\midrule
        %scalability & ~ & ~ & ~ & ~ & ~ \\
        %privacy & ~ & ~ & ~ & ~ & ~ \\
         \bottomrule
    \end{tabular}
    }
\end{table}
\end{landscape}


%Privacy pass notes:
%tokens: blinded tokens (section 2.4 paper)
%proofs: DLEQ (section 3.2 paper)
%signing: some MAC
%time:
%data:

%black box accumulators:
%tokens:  SXDH commitment scheme
%proofs: Groth Salai proofs
%signature: structure preserving signatures
%elliptic curves: BN (paper section 4.3)
%time (issue): 36ms (token size 3kb)
%time (accumulate points): 268 ms (token size 2kb)
%time (verification): 256 ms (output single bit)
%data: see above

%BBA+:
%tokens: shrinking structure-preserving trapdoor commitments~\cite{EC:AKOT15}
%proofs: Groth-Sahai proofs
%signature: Structure Preserving Signatures~\cite{C:AGHO11}
%elliptic curves: (section 6.1) Fp254BNb BN curves, Fp254n2BNb, Ate pairing
%time (issue): 115ms  data(issue): send: 672 bytes, received: 320 bytes
%time (accumulate):  386 ms, data(acc): send: 3728 bytes, received: 320 bytes
%time (verify):  376 ms, data(ver): send: 3664 bytes, received: 320 bytes

% BBW
% tokens: TODO
%proofs: Bulletproofs~\cite{SP:BBBPWM18}, $\Sigma$ proofs
%signature: TODO
%elliptic curves: curve25519~\cite{PKC:Bernstein06}
%time (issue): TODO
%time (accumulate):  TODO
%time (verify):  TODO

==> defs.tex <==
\def\authnotes{1}
\newcommand{\authnote}[2]{\ifnum\authnotes=1\begin{quote}\textbf{#1 says:} #2\end{quote}\fi}
\newcommand{\authfnote}[2]{\ifnum\authnotes=1\footnote{\textbf{#1 says:} #2}\fi}

\newcounter{mynote}[section]
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{darkmagenta}{rgb}{0.55, 0.0, 0.55}
\definecolor{darkpink}{rgb}{0.86,0.44,0.58}
\newcommand{\notecolor}{blue}
\newcommand{\nnote}[1]{\ifnum\authnotes=1\refstepcounter{mynote}{\bf \textcolor{darkmagenta}{$\ll$Sofia~\thenote: {\sf #1}$\gg$}}\fi}


==> protocol.tex <==
\section{The \protocolname Protocol}\label{sec:protocol}
In the following, we give a high-level description of how the \protocolname protocol 
works. The protocol follows a modular approach, allowing to interchange several of the 
building blocks without necessarily diminishing security/privacy properties. However, 
using the right components allows for a highly efficient protocol that improves 
latency, scalability, and allows to reduce the number of zero-knowledge proofs.  

\subsection{Desired Privacy-Properties}
Consecutively, we give some details about the security model an the desired 
privacy-properties that we require the \protocolname protocol to achieve. We argue that 
these properties are essential for a privacy-preserving operation of our protocol. From 
a broad perspective these privacy properties include 
\begin{itemize}
    \item \emph{Unlinkability} of different incentives between categories, between 
    individual personalised preferences and unlinkability of the payment tokens to 
    certain incentive interactions.
    \item \emph{Anonymity} of users interacting with the incentive system when sharing 
    private metrics with the issuer of the incentive system and providers of the 
    incentives. 
    \item \emph{Public Verifiability} of the correct execution of the protocol and 
    validation of the zero-knowledge proofs for the correct reward computation for 
    interacting with the incentive system. 
\end{itemize}

\subsubsection{Unlinkability} Pfitzmann and Köhntopp~\cite{Pfitzmann2001} introduced 
the concept of unlinkability, which refers to the ability to prevent the linkage of 
different activities or information across contexts. It ensures that data or actions in 
one context cannot be connected or traced to the same data or actions in another 
context, preserving privacy and anonymity. Unlinkability safeguards against correlation 
and linkage, maintaining confidentiality and protecting sensitive information.

\begin{definition}[Unlinkability]
Two or more items (i.e. subjects, objects or actions) are unlinkable, if an adversary 
cannot successfully distinguish if those items are related to each other.
\end{definition}

In the \protocolname protocol, we want to ensure that two or more incentives cannot be 
linked together. Moreover, if the incentives belong to a broader category, it should 
not be possible to link those incentives together. Additionally, it is also of interest 
to personalise incentives, which again should not be able to be linked to a specific 
user or that they are related. Likewise, we require that an users interaction of any 
kind with the incentive should not be able to be linked to the particular user. 
Finally, when an user is rewarded for interacting with the incentive system, it should 
not be possible to link the user to the payment. 

\subsubsection{Anonymity} In the definition of Pfitzmann and 
Köhntopp~\cite{Pfitzmann2001}, a subject is called anonymous if an adversary cannot 
successfully identify the subject within a set of subjects. A notation that is more 
often used in practice is the definition of $k$-anonymity introduced by Samarati and 
Sweeney~\cite{samarati-protect}. K-anonymity ensures that each individual in a dataset 
cannot be distinguished from at least $k-1$ other individuals based on certain 
identifying attributes. It aims to protect privacy by making it challenging to identify 
specific individuals within the dataset, mitigating the risk of re-identification.   

\begin{definition}[$k$-Anonymity]
$k$-anonymity guarantees that an individuals data in a sanitised dataset is 
indistinguishable from the data of at least $k-1$ other individuals, whose data is 
within the original dataset. Thus, each quasi-identifying tuple in the sanitised 
dataset occurs at least $k$ times. 
\end{definition}

In the \protocolname protocol, we want to provide private metrics to the issuer and the 
different providers for the incentives. We require that any metrics shared are 
protected by $k$-anonymity. This can practically be achieved by using a 
privacy-preserving threshold aggregation reporting system such as 
STAR~\cite{CCS:DSQGLH22}. 

\subsubsection{Public Verifiability} While there does not exist a formal definition of 
public verifiability per se, we still require public verifiability of the protocol in 
several places. In general, we refer with public verifiability to the ability to 
publicly verify the correctness and integrity of certain operations and procedures 
within our protocol.

This includes that we require that the interaction state changes of an user interacting 
with the incentive system should be verifiable by the issuer. Moreover, we require that 
the compensation for interacting with the incentive system in form of a reward, and 
therefore the correct interaction with the incentives, should be public verifiable 
using smart contracts on a L1 blockchain. Finally, we require that the zero-knowledge 
proofs for the rewards computation and identity proof can be publicly validated and are 
complete, sound and should not reveal any information about the statement to be proven, 
i.e. they should be zero-knowledge.   

\subsection{Building Blocks}
We follow a modular approach using different building blocks that can easily be 
interchanged without compromising the security and privacy properties, but also to 
ensure adaptability and efficient implementation on various platforms. 

\subsubsection{Black Box Accumulators} 
Cryptographic accumulators are used as an efficient data structure for the 
cryptographic tokens. These tokens are used to encapsulate the interaction state of the 
incentive system in a privacy preserving manner. Furthermore, they prevent linking user 
interactions within the incentive system.

\subsubsection{Zero-Knowledge Proofs}
In various places in the protocol, zero-knowledge proofs are used to synchronise the 
state of the interaction with the incentives between the user and the issuer. Notably, 
we use zero-knowledge proofs in the \protocolname protocol for the verification of the 
black box accumulator, for computing a proof that the incentives have been correctly 
computed and a proof that the customers wallet has been KYC'ed. 

While we do not want to restrict the use of any particular zero-knowledge proof system, 
we want to highlight certain recommendations to ensure an efficient interplay between 
the other building blocks of the protocol. Accordingly, as zero-knowledge proof systems 
with a trusted setup usually introduce risks due to trust dependencies, lack of 
transparency, long-term security concerns and scalability issues we prefer a proof 
system without the need of a trusted setup. Besides, we want to avoid the use of proof 
systems that require pairing-based cryptography as this usually introduces computation 
overhead, implementation complexity and requires specific elliptic curves that limit 
interoperability and adoption. 

\subsubsection{Smart Contracts}
Public verifiability of the incentive computation is achieved by performing the 
verification of the zero-knowledge proofs on-chain. Hereby, smart contracts are 
leveraged running on a L1 blockchain. The smart contracts must be able to support the 
cryptographic operations needed to perform the verification of the zero-knowledge 
proofs and additionally should handle the settlement for the payment of the incentive 
system. 

\subsection{\protocolname protocol}
The \protocolname protocol consist of a set of two protocols, where the first protocol 
describes the interaction of the user with the incentive system and the synchronisation 
of the interaction with the issuer. The second protocol is designed to specify the 
local calculation of the rewards that a user earns when interacting with the incentive 
system, and the corresponding public validation of the correct reward calculation by 
using a L1 blockchain. 

\subsubsection{Interaction with Incentives} 
The first protocol is designed to specify the interaction of the user with the issuer 
of the incentive scheme. Therefore, we define an interaction state, that keeps track of 
the interaction over time. We implement the interaction state using a cryptographic 
token, more specifically using black box accumulators (BBAs). More details about the 
BBAs is explained in Section~\ref{sec:bba}.

\begin{figure}[htb!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/sequence-bba.pdf}
    \caption{The first protocol defines the interaction of the user with the incentive 
    system by the issuer. We use black box accumulators to keep track of the 
    interaction over time. Additionally, a zero knowledge proof is used to synchronise 
    the black box accumulator between the user and the issuer.}
    \label{fig:bba}
\end{figure}

The protocol used to interact with the incentives using the BBA data structure is 
illustrated as sequence diagram in Figure~\ref{fig:bba}. The workflow of the protocol 
is as follows:
\begin{itemize}[leftmargin=4em]
    \item [\circled{1}] Initially, the user initialises the BBA. The interaction state 
    is initialised to an all zero-vector. This step has do be done only once per 
    payment cycle. 
    \item [\circled{2}] The user then makes a commitment \texttt{com} to the BBA, and 
    generates a zero-knowledge proof $\pi$ confirming the initial state of the BBA. 
    This commitment and the proof are then sent via an anonymous channel (e.g. by using 
    OHTTP) to the issuer.
    \item [\circled{3}] The issuer performs some anti-fraud checks verifying that it is 
    a legitimate user request.
    \item [\circled{4}] The issuer stores the id of the BBA to keep track of the 
    current active BBAs. 
    \item [\circled{5}] The user than interacts with the incentive system. The 
    interaction is stored locally within the BBA by updating the corresponding counter 
    values.
    \item [\circled{6}] In regular intervals, the user synchronises the BBA with the 
    issuer of the incentive system. 
    \item [\circled{7}] To synchronise the BBA with the issuer, the user again makes a 
    commitment \texttt{com} to the current state of the BBA, and generates a 
    zero-knowledge proof $\pi$ confirming the actual updated state of the BBA. The 
    request is sent over \texttt{OHTTP} in order to ensure \textit{privacy} and 
    \textit{unlinkability}. 
    \item [\circled{8}] The issuer performs some anti-fraud checks verifying that it is 
    a legitimate user request.
    \item [\circled{9}] Finally, the issuer verifies the zero-knowledge proof $\pi$ and 
    synchronises the BBA identified by its id.
\end{itemize}

\noindent
Note, steps \circled{5} to \circled{9} can be repeated several times, while steps 
\circled{1} to \circled{4} are only executed once, and the BBA is retained until the 
user redeems its incentives by initiating a reward request. 

\subsubsection{Reward calculation and Validation} 
The second protocol is designed to specify how users can be rewarded for their 
participation in the incentive system and the public verification of the reward 
computation. It assumes, that an user has initiated a black box accumulator, and 
interacted with the incentive system. The user than computes its rewards, for 
interacting with the incentive system, locally on device and additionally computes two 
zero-knowledge proofs to confirm a correct rewards computation and to confirm that the 
user has a KYCed wallet. The purpose of the second zero-knowledge proof of a KYCed 
wallet, also referred to as identity proof, is to reduce the amount of fraudulent users 
in the incentive system. More details about the zero-knowledge proofs are discussed in 
Section~\ref{sec:zkp}. 

Furthermore, to achieve public verifiability of the rewards proofs, the verification of 
the zero knowledge proofs is done on-chain using smart contracts on a L1 blockchain. 
The details and challenges of verifying zero knowledge proofs in a smart contract are 
further discussed in Section~\ref{sec:blockchain}. 

We outline the protocol for rewards calculation and validation using a public 
blockchain in a sequence diagram in Figure~\ref{fig:reward}. The protocol is works as 
follows:

\begin{itemize}[leftmargin=4em]
    \item [\circled{1}] We assume that the user has interacted with the incentive 
    system and the BBA is updated by the issuer reflecting the interaction. 
    \item [\circled{2}] The user initiates the reward protocol, by calculating the 
    rewards according to the state of the BBA. 
    \item [\circled{3}] Next, the user generates a zero-knowledge proof of reward 
    calculation. 
    \item [\circled{4}] Additionally, the user adds a zero-knowledge proof of identity.
    \item [\circled{5}] The user requests an on-chain settlement, revealing the BBA and 
    the two zero-knowledge proofs of reward calculation and identity. 
    \item [\circled{6}] A smart contract running on a L1 blockchain is triggered, and 
    the proofs for a correct reward calculation and the proof for the identity are 
    verified. 
    \item [\circled{7}] The smart contract also performs several anti-fraud checks, 
    verifying that the reward request is legitimate. 
    \item [\circled{8}] Finally, the user receives payment tokens.  
\end{itemize}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=.5\textwidth]{figures/sequence-blockchain.pdf}
    \caption{The second protocol for the local reward computation based on the black 
    box accumulators issued during interacting with the incentive system. The reward 
    computation is accompanied by two zero knowledge proofs of correct reward 
    computation and a identity proof of a KYCed wallet. The verification of the zero 
    knowledge proofs is performed in a smart contract on-chain to allow for public 
    verifiability.}
    \label{fig:reward}
\end{figure}


==> verifiability.tex <==
\section{Public verifiability}
\label{sec:zkp}

A BBA-based system cannot be only used to accumulate transaction tokens, but it can be also used for any other type of interaction.
~\cite{DBLP:journals/corr/abs-2106-01940}, for example, mentions that it can be used in a digital advertising setting where users are ``rewarded'' depending on how many points they have accumulated (how many digital ads, they have watched).
As said, one of these ideas is that of compensating users that view ads is not so far-fetched: Brave Ads~\cite{bravebat}, for example, compensates users that view ads with cryptocurrency in their built-in browser wallet.

During the spending procedure, users signal to \VF which and how many points they want to spend and get a reward for.
They send these values to \VF (in the form of $v$s, the spending vector), where they can calculate the rewards.
For this, the \TTP first makes public (or alternatively makes it only private to the \IS and \VF) a policy vector and a commitment to it where each index corresponds to an accumulation issuer and each value sets the ammount each point is worth for each accumulation issuer.
Rewards are then computed by \VF by calculating the scalar product between the spending vector and the policy vector.
For example, if the spending vector at the time of reward computation was:

$$
\stsp = [0,1,3,5,0,0]
$$ and the policy vector is defined as
$$
\stpl = [3,5,2,3,3,2]
$$

the reward will be:

\begin{equation}\label{eq:reward}
\begin{aligned}
\strw &= \langle \stsp, \stpl \rangle \\
&= 0 \times 3 + 1 \times 5 + 3 \times 2
+ 5 \times 3 + 0 \times 3 + 0 \times 2 \\
&= 26.
\end{aligned}
\end{equation}

In order to be able to verify that \strw was computed correctly, \VF additionally generates a zero-knowledge proof that the computation of \strw indeed is the scalar product of \stsp and \stpl.
Additional proofs might be needed from \U side: if the rewards is a fiat-currency, they might want to prove that their wallet have been verified with a KYC provider, which allows to perform anti-fraud checks.
This can be done via a ring signature where authorised users are part of a public ring.
In the \protocolname protocol we do not strictly require any particular KYC scheme; however, we outline a possible solution for this in Appendix~\ref{appendix:identityproof}.

\subsection{Rewards Proof}

For a rewards proof, we need to proof the following:

\begin{enumerate}
  \item That \U is an authorised user of the system via a ring signature.
  \item That the reward calculation was correct and in a correct range.
\end{enumerate}

One of the most important steps for getting rewards is to prove to \VF{} that \U is an authorised user of the system.
This can be done via a ring-signature scheme where the identity is authorised but protected by a degree of anonimity.
\sofia{we need to define the scheme and reason why only here we need to disclose the identity.}

In order to perform the reward calculation, $\pi_{reward}$, as noted, in the \protocolname{} protocol, we use zero-knowledge proofs to attest the correctness of the reward computation.
We specifically need to prove that the inner product relation between $\stsp$ and $\stpl$ as outlined in Equation~\ref{eq:reward} was done correctly.
Note that for this we require to generate a multi-commitment to $\stsp$ (which we call $C_{\stsp} = g^{\stsp}$) and a multi-commitment to $\stpl$ (which we call $\stpl = h^{\stpl}$), where \VF{} will perform the inner-product multiplication as $c = \langle \stsp, \stpl \rangle$.
Following~\cite{SP:BBBPWM18} with proofs for inner-product arguments (first introduced by~\cite{EC:BCCGP16}), we then have $P = C_{\stsp} C_{\stsp} \cdot u^{\langle \stsp, \stpl \rangle}$, where $u \in \mathbb{G}$, which is a binding commitment to $\stsp$ and $\stpl$.
One also proves that the sum of all values in \stsp{} does not exceed a limit $L$ set by \IS{} by using a `Inner-Product Range Proof'.
This is done by $C_{\stsp} = g^{\stsp}$
Hence, the relation we prove is:

\[\mathcal{R} = \{(((g, h) \in mathbb{G}^n, (u, P) \in \mathbb{G}), C_{\stsp}; (a,b))\ |\ P = g^a h^b \cdot u^{\langle a, b \rangle} \land c = \langle a, b \rangle\} \leq L.\]

For the relation $\mathcal{R}^{\texttt{reward}}$, we use a \emph{range proof} to show that the sum of the incentives does not exceed the limit $L$.
As the $\emph{policy vector}$ is public, we can use a lightweight Bulletproof that was introduced by Gentry et. al.~\cite{EC:GenHalLyu22} to prove that the reward is the inner product of the state and the policy vector.

\paragraph{Limitations.} When computing the rewards proof \U's id is protected by an anonimity set that provides anonimity depending on the size of the set.
The only information that is learned by \VF{} is the actual reward computation.
We assume that at this point it is fine to leak that information, but \VF remains oblivious to how many incentives interactions \U still holds.
Note that we have yet to arrive to public verifiability of the rewards computation.
A potential solution for that is to do the proof verification on a public blockchain.
Though, verifying zero-knowledge proofs on a public blockchain introduces additional challenges in terms of scalability, computational effort and communication.% complexity. %More details are discussed in
%Section~\ref{sec:blockchain}.

%\todo[inline]{Detailed math writeup of bulletproofs -> \url{https://doc-internal.dalek.rs/bulletproofs/notes/inner_product_proof/index.html}}
%\url{https://cathieyun.medium.com/building-on-bulletproofs-2faa58af0ba8}
%\url{https://dankradfeist.de/ethereum/2021/07/27/inner-product-arguments.html}

